Noncommutative Geometry and Gauge theories on AF algebras

Non-commutative geometry (NCG) is a mathematical discipline developed in the 1990s by Alain Connes. It is presented as a new generalization of usual geometry, both encompassing and going beyond the Riemannian framework, within a purely algebraic formalism. Like Riemannian geometry, NCG also has links with physics. Indeed, NCG provided a powerful framework for the reformulation of the Standard Model of Particle Physics (SMPP), taking into account General Relativity, in a single "geometric" representation, based on Non-Commutative Gauge Theories (NCGFT). Moreover, this accomplishment provides a convenient framework to study various possibilities to go beyond the SMPP, such as Grand Unified Theories (GUTs). This thesis intends to show an elegant method recently developed by Thierry Masson and myself, which proposes a general scheme to elaborate GUTs in the framework of NCGFTs. This concerns the study of NCGFTs based on approximately finite $C^*$-algebras (AF-algebras), using either derivations of the algebra or spectral triples to build up the underlying differential structure of the Gauge Theory. The inductive sequence defining the AF-algebra is used to allow the construction of a sequence of NCGFTs of Yang-Mills Higgs types, so that the rank $n+1$ can represent a grand unified theory of the rank $n$. The main advantage of this framework is that it controls, using appropriate conditions, the interaction of the degrees of freedom along the inductive sequence on the AF algebra. This suggests a way to obtain GUT-like models while offering many directions of theoretical investigation to go beyond the SMPP.

==> tex_open/ResumFr.tex <==
\chapter*{Résumé}
\addcontentsline{toc}{chapter}{Résumé}
 

\vspace{0.5cm}
La géométrie non commutative est un cadre puissant pour reformuler le modèle standard de la physique des particules (SMPP) en tenant compte la relativité générale, en une seule représentation "géométrique" basée sur les théories des champs de jauge non commutatives (NCGFT). Cette réalisation ouvre la porte à l'étude de nombreuses possibilités de construire de nouveaux modèles au-delà de la SMPP, comme les théories de jauge grands unifiées (GUT). Cette thèse cherche à montrer une méthode élégante récemment développée par Thierry Masson et moi-même qui propose un schéma général pour construire des GUT dans le domaine des NCGFT. Ceci concerne les NCGFT basées sur les C-algebres Approximativement Finies (AF) en utilisant soit les dérivations de l'algèbre, soit des triples spectraux. La séquence inductive définissant l'algèbre AF est utilisée pour permettre la construction d'une séquence de NCGFT de types Yang-Mills Higgs. Le principal avantage de ce cadre est de contrôler, à l'aide de conditions adéquates, l'interaction des degrés de liberté le long de la séquence inductive sur l'algèbre AF, et de suggérer un moyen de d'obtenir des modèles de type GUT similaires à celui de Georgi-Glashow. 
\begin{itemize}
\item utilise mes résumés déjà faits
\item sert pour strasbourg et CV.. 10 pages
\end{itemize}


==> tex_open/affidavit.tex <==
 
\newpage
 
\chapter*{Affidavit}					
%\addcontentsline{toc}{chapter}{Affidavit}
 
\iftrue % Déclaration sur l'honneur pour une thèse en français (inverser les \if pour une thèse en anglais)
      Je soussigné, Gaston Nieuviarts, %% Prénom et Nom de l'auteur %%
    déclare par la présente que le travail présenté dans ce manuscrit est mon propre travail, réalisé sous la direction scientifique de Thierry Masson, % Prénom et Nom du directeur de thèse et s’il y a lieu du co-directeur de thèse
    dans le respect des principes d’honnêteté, d'intégrité et de responsabilité inhérents à la mission de recherche. Les travaux de recherche et la rédaction de ce manuscrit ont été réalisés dans le respect à la fois de la charte nationale de déontologie des métiers de la recherche et de la charte d’Aix-Marseille Université relative à la lutte contre le plagiat.
    
    Ce travail n'a pas été précédemment soumis en France ou à l'étranger dans une version identique ou similaire à un organisme examinateur.
    
    Fait à Marseille le 15/09/2022.
    
    \begin{flushright}\includegraphics[width=120px,height=40px]{logo/sign.png}\end{flushright}% signature
\fi

\iffalse % Affidavit of Honour for english thesis (invert the \if for an English thesis)
    I, undersigned, [First Name Surname], %% First Name and Surname of the PhD student
    hereby declare that the work presented in this manuscript is my own work, carried out under the scientific direction of [First Name Surname], %% First Name and Surname of the thesis director and if applicable of the co-thesis director
    in accordance with the principles of honesty, integrity and responsibility inherent to the research mission. The research work and the writing of this manuscript have been carried out in compliance with both the french national charter for Research Integrity and the Aix-Marseille University charter on the fight against plagiarism.
    
    This work has not been submitted previously either in this country or in aother country in the same or in a similar version to any other examination body.\\
    
    [Place] [date]
    
    \begin{flushright}\includegraphics[width=120px,height=40px]{example-image-b}\includegraphics[width=40,height=15px]{example-image-a}\end{flushright} % signature
\fi

~\vfill
\begin{center}
	\begin{minipage}[c]{0.25\linewidth}
		\includegraphics[height=35px]{logo/by-nc-nd-eu}
	\end{minipage}\hfill
\end{center}

Cette \oe{}uvre est mise à disposition selon les termes de la \href{https://creativecommons.org/licenses/by-nc-nd/4.0/deed.fr}{Licence Creative Commons Attribution - Pas d’Utilisation Commerciale - Pas de Modification 4.0 International}. % consultez les conditions de la licence cc by-nc-nd, vous pouvez appliquer une licence moins restrictive, cc by-nc-sa par exemple
 

==> tex_open/gloss.tex <==
%%% Acronymes

\newacronym{bc}{BC}{band contrast}

\newacronym{asb}{ASB}{bande de cisaillement adiabatique --ou \emph{Adiabatic Shear Band}--}


%%% Définitions (glossaire standard)

\newglossaryentry{rutile}{
	name={rutile},
	description={Espèce minérale composée de dioxyde de titane (\ce{TiO2}) et de traces de fer},
	}
	

%%% Nomenclature	

\newglossaryentry{+a}{
  type=notation,
  name={$+a$},
  description={Opérateur},
  sort={aaa}
}

\newglossaryentry{2a}{
  type=notation,
  name={$2a$},
  description={Nombre},
  sort={aab}
}

\newglossaryentry{ca}{
  type=notation,
  name={$:a$},
  description={Symbole de ponctuation},
  sort={aac}
}

\newglossaryentry{Aa}{
  type=notation,
  name={$Aa$},
  description={Lettre majuscule},
  sort={aad}
}

\newglossaryentry{aa}{
  type=notation,
  name={$aa$},
  description={Lettre minuscule},
  sort={aae}
}

\newglossaryentry{alpha}{
  type=notation,
  name={$\alpha$},
  description={Lettre grecque},
  sort={aaf}
}

